Bidirectional Consistency Models

Diffusion models (DMs) are capable of generating remarkably high-quality samples by iteratively denoising a random vector, a process that corresponds to moving along the probability flow ordinary differential equation (PF ODE). Interestingly, DMs can also invert an input image to noise by moving backward along the PF ODE, a key operation for downstream tasks such as interpolation and image editing. However, the iterative nature of this process restricts its speed, hindering its broader application. Recently, Consistency Models (CMs) have emerged to address this challenge by approximating the integral of the PF ODE, largely reducing the number of iterations. Yet, the absence of an explicit ODE solver complicates the inversion process. To resolve this, we introduce Bidirectional Consistency Model (BCM), which learns a single neural network that enables both forward and backward traversal along the PF ODE, efficiently unifying generation and inversion tasks within one framework. We can train BCM from scratch or tune it using a pretrained consistency model, which reduces the training cost and increases scalability. We demonstrate that BCM enables one-step generation and inversion while also allowing the use of additional steps to enhance generation quality or reduce reconstruction error. We further showcase BCM's capability in downstream tasks, such as interpolation and inpainting. Our code and weights are available at https://github.com/Mosasaur5526/BCM-iCT-torch.

==> res.tex <==
\begin{figure}[t]
  \centering
    \begin{minipage}[b]{0.72\textwidth}
    \centering
\begin{minipage}[b]{\textwidth}
  \captionof{table}{Sample quality on CIFAR-10. $^*$Results estimated from Figure 13 in \citet{kim2023consistency}. $^\dag$For our BCM and BCM-deep, we use ancestral sampling when NFE=2, zigzag sampling when NFE=3, and the combination of both when NFE=4. 
Our results indicate that ancestral and zigzag sampling can individually improve FID, and their combination can achieve even better performance.}\label{tab:generation-result}
    \scalebox{0.88}{
\begin{tabular}{@{}lccc@{}}
\toprule
\textsc{METHOD}                                              & \textsc{NFE} ($\downarrow$) & \textsc{FID} ($\downarrow$) & \textsc{IS} ($\uparrow$) \vspace{2pt}\\
\multicolumn{4}{@{}l@{}}{\textbf{Diffusion with Fast Sampler /  Distillation}}            \\ \toprule
DDIM \citep{song2020denoising}                                          & 10     & 8.23     &           -  \\
DPM-solver-fast \citep{lu2022dpm}                                     & 10     &   4.70    &     -          \\
AMED-plugin \citep{zhou2023fast}                                   & 5       & 6.61     & - \\
Progressive Distillation \cite{salimans2021progressive}                              & 1     &   8.34    &         8.69       \\
\multirow{2}{*}{CD (LPIPS) \cite{song2023consistency}}                          & 1     &   3.55    & 9.48              \\
                                                     & 2     &    2.93   & 9.75 \\

\multirow{2}{*}{CTM (LPIPS, GAN loss) \cite{kim2023consistency}    }                                 & 1     &  1.98     &  -            \\
                                                     & 2     &  1.87     &  -   
                                                       \\
CTM (LPIPS, w/o GAN loss) \cite{kim2023consistency}                                     & 1     &  $>5.00^*$     &  -            \\     
\vspace{-6pt}\\
\textbf{Direct Generation}                           &       &       &               \\ \toprule
Score SDE (deep) \cite{song2020score}                                    & 2000     &   2.20    &  9.89             \\
DDPM \citep{ho2020denoising}                                            & 1000     &   3.17    &  9.46             \\
EDM \cite{karras2022elucidating}                                                & 35     &  2.04     &  9.84              \\
\multirow{2}{*}{CT (LPIPS) \cite{song2023consistency}    }                                 & 1     &  8.70     &  8.49            \\
                                                     & 2     &  5.83     &  8.85             \\
CTM (LPIPS, GAN loss) \cite{kim2023consistency}                                     & 1     &  2.39     &  -            \\
\multirow{2}{*}{iCT \cite{song2023improved}}                                 & 1     &  2.83     &  9.54             \\
                                                     & 2     &  2.46     &  9.80             \\
\multirow{2}{*}{iCT (deep) \cite{song2023improved}}                          & 1     &  2.51     &  9.76             \\
                                                     & 2     &  2.24     &  9.89             \\ \midrule
\multirow{4}{*}{\textbf{BCM (ours)}$^\dag$   }                             & 1     & 3.10      &  9.45             \\
                                                     & 2     & 2.39      &  9.88             \\
                                                     & 3     & 2.50      &  9.82             \\
                                                     & 4     & 2.29      &  9.92             \\
\multirow{4}{*}{\textbf{BCM (ours, deep)}$^\dag$}           & 1     &  2.64     &  9.67             \\
                                                     & 2     &  2.36     &  9.86             \\
                                                     & 3     &  2.19     &  9.94             \\
                                                     & 4     &  2.07     &  10.02             \\ \bottomrule
\end{tabular}
}{\vspace{0.1cm}}
\end{minipage}
    \end{minipage}
    \hspace{5pt}
     \begin{minipage}[b]{0.248\textwidth}
     \centering
    \begin{minipage}[b]{\textwidth}
    \includegraphics[width=\textwidth]{Figures/generation/onestep-deep-main.png}
     \text{\ \ \ \ \ \ \ \ \ \small (a) 1-step (FID 2.64)}
   \end{minipage}
    \begin{minipage}[b]{\textwidth}
    \includegraphics[width=\textwidth]{Figures/generation/twostep-deep-main.png}
     \text{\ \ \ \ \ \ \ \ \ \small (b) 2-step (FID 2.36)}
   \end{minipage}
   \begin{minipage}[b]{\textwidth}
    \includegraphics[width=\textwidth]{Figures/generation/threestep-deep-main.png}  \text{\ \ \ \ \ \ \ \ \ \small (c) 3-step (FID 2.19)}
   \end{minipage}
   \begin{minipage}[b]{\textwidth}
    \includegraphics[width=\textwidth]{Figures/generation/fourstep-deep-main.png}   \text{\ \ \ \ \ \ \ \ \ \small (d) 4-step (FID 2.07)}
   \end{minipage}
    \captionof{figure}{Uncurated samples by BCM-deep. We can see our sampling methods improve the FID while largely preserving the content.}\label{fig:samples_main_text}
     \end{minipage}
\vspace{-10pt}
\end{figure}

